HAL3D: Hierarchical Active Learning for Fine-Grained 3D Part Labeling

We present the first active learning tool for fine-grained 3D part labeling, a problem which challenges even the most advanced deep learning (DL) methods due to the significant structural variations among the small and intricate parts. For the same reason, the necessary data annotation effort is tremendous, motivating approaches to minimize human involvement. Our labeling tool iteratively verifies or modifies part labels predicted by a deep neural network, with human feedback continually improving the network prediction. To effectively reduce human efforts, we develop two novel features in our tool, hierarchical and symmetry-aware active labeling. Our human-in-the-loop approach, coined HAL3D, achieves 100% accuracy (barring human errors) on any test set with pre-defined hierarchical part labels, with 80% time-saving over manual effort.

==> tables/ablation.tex <==
% \begin{table}[t!]
% \begin{center}
% \caption{ Ablation study of key designs in our method for chair category.}
% \label{tab:ablation}
% \begin{tabular}{ |c|c|c|c|c|c| } 
% \hline
% Ablations & PV & FV & PV/M & PM & T \\
% \hline
% w/o-DL & 0 & 0 & 0 & 6643 & 22.05\\ 
% w/o-AL & 0 & 0 & 4481 & 2162 & 8.65\\ 
% w/o-Hier & 540 & 101 & 4296 & 1301 & 5.99\\ 
% w/o-Sym & 5585 & 702 & 6009 & 2031 & 5.21\\ 
% Ours & 5679 & 647 & 5440 & 1473 & 4.34\\ 
% \hline
% \end{tabular}
% \end{center}
% \end{table}

\begin{table}[t!]
\begin{center}
\caption{Ablation study on key modules of HAL3D for chair category. The last column ``Lab.~time" denotes total labeling time.}
\label{tab:ablation}
\begin{tabular}{c|ccc|c} 
\hline
Row ID &Prop. & Hier. & Sym. & Lab. time$\downarrow$ (h) \\
\hline \hline
2nd &- & - & - &  22.05\\
3rd &\checkmark & - & - &  8.65\\
4th &\checkmark & - & \checkmark &  5.99\\
5th &\checkmark & \checkmark & - &  5.21\\
6th &\checkmark & \checkmark & \checkmark &  {\bf 4.34} \\
\hline
\end{tabular}
\end{center}
\end{table}

==> tables/abo_compare_acc.tex <==
% \begin{table}[t!]
% \begin{center}
% \caption{ Comparison for different methods to pass human verification on test set of ABO.}
% \label{tab:abo_comparison}
% \begin{tabular}{ |c|c|c|c|c|c|c| } 
% \hline
%  & Methods & PV & FV & PV/M & PM & T \\
% \hline
% \multirow{3}{3em}{Chair} &PartNet & - & - & 512	& 8459&28.25\\ 
% &NGSP & - & - & 495 & 8476 & 28.30\\
% &Ours & 5234 & 844 & 9516 & 2363 & 6.46 \\ 
% \hline
% \multirow{3}{3em}{Table} &PartNet & - & - & 144 & 8292 & 33.94\\ 
% &NGSP & - & - & 42 & 8394 & 34.32\\
% &Ours & 4547 & 584 & 8532 & 2673 & 7.41 \\ 
% \hline
% \multirow{3}{3em}{Lamp} &PartNet & - & - & 41 & 9874 & 31.53\\ 
% &NGSP & - & - & 28 & 9887 & 31.56\\
% &Ours & 1044 & 383 & 7846 & 1669 & 4.38 \\ 
% \hline
% \multirow{3}{3em}{Cabinet} &PartNet & - & - & 26 & 5099 & 13.35
%  \\ 
% &NGSP & - & - & 79 & 5046 & 13.22 \\
% &Ours & 863	& 215& 5091& 1289& 3.34\\ 
% \hline
% \multirow{3}{3em}{Bed} &PartNet & - & - & 184 & 10581 & 25.02\\ 
% &NGSP & - & - & 240 & 10525 & 24.90\\
% &Ours & 6500& 394& 9628 & 1263 & 4.51
% \\ 
% \hline
% \end{tabular}
% \end{center}
% \end{table}

\begin{table}[t!]
\begin{center}
\caption{Labeling accuracy comparison on ABO.}
\label{tab:abo_comparison_new}
\begin{tabular}{ l|c|c|c|c|c } 
\hline
 & Chair & Table & Lamp & Cabinet & Bed \\
\hline
PartNet+mod. & 88.96	& 86.51 & 90.91 & 90.24 & 89.37\\
\hline
NGSP+mod. & 88.77 & 86.40 & 91.37 & 90.56 & 89.93\\
\hline
HAL3D & {\bf 93.07} & {\bf92.55} & {\bf96.29} & {\bf94.48} & {\bf93.71} \\
\hline
\end{tabular}
\end{center}
\vspace{-15pt}
\end{table}

==> tables/al_acc.tex <==
\begin{table}[t!]
\begin{center}
\caption{ Active learning accuracy analysis on fine-grained part labeling.}
\label{tab:al_acc}
\begin{tabular}{ |c|c|c|c|c|c|c| } 
\hline
 & Methods & PV & FV & PV/M & PM & T \\
\hline
\multirow{3}{3em}{Chair} &PartNet & - & - & 512	& 8459&28.25\\ 
&NGSP & - & - & 495 & 8476 & 28.30\\
&Ours & 5234 & 844 & 9516 & 2363 & 6.46 \\ 
\hline
\multirow{3}{3em}{Table} &PartNet & - & - & 144 & 8292 & 33.94\\ 
&NGSP & - & - & 42 & 8394 & 34.32\\
&Ours & 4547 & 584 & 8532 & 2673 & 7.41 \\ 
\hline
\multirow{3}{3em}{Lamp} &PartNet & - & - & 41 & 9874 & 31.53\\ 
&NGSP & - & - & 28 & 9887 & 31.56\\
&Ours & 1044 & 383 & 7846 & 1669 & 4.38 \\ 
\hline
\multirow{3}{3em}{Cabinet} &PartNet & - & - & 26 & 5099 & 13.35
 \\ 
&NGSP & - & - & 79 & 5046 & 13.22 \\
&Ours & 863	& 215& 5091& 1289& 3.34\\ 
\hline
\multirow{3}{3em}{Bed} &PartNet & - & - & 184 & 10581 & 25.02\\ 
&NGSP & - & - & 240 & 10525 & 24.90\\
&Ours & 6500& 394& 9628 & 1263 & 4.51
\\ 
\hline
\end{tabular}
\end{center}
\end{table}


==> tables/dataset.tex <==
\begin{table}[t!]
\begin{center}
\caption{ The statistics of our dataset.\ym{Maybe we can move this table to supp}}
\label{tab:datasets}
\begin{tabular}{ |c|c|c|c|c|c|c| } 
\hline
Dataset & Splits & Chair & Table & Lamp & Cabinet & Bed\\
\hline
Labels & - & 29 & 41 & 27 & 18 & 14\\ 
\hline
\multirow{3}{3em}{PartNet} & Train & 50 & 50 & 50 & 50& 44\\ 
& val & 50 & 50 & 50 & 50& -  \\ 
& test & 400 & 400 & 400 & 400& - \\ 

\hline
ABO & test & 800 & 400 & 200 & 400 & 400\\ 

\hline
\end{tabular}
\end{center}
\end{table}

==> tables/node_analysis.tex <==
\begin{table}[t!]
\begin{center}
\caption{Statistics for active learning at different nodes of our hierarchical design and non hierarchical setting up.}
\label{tab:node_analysis}
\begin{tabular}{ |c|c|c|c|c|c|c| } 
\hline
Data & L & PV & FV & PV/M & PM & T \\
\hline
w/o-Hier & 29 & 540 & 101 & 4296 & 1301 & 5.99\\ 
\hline
Chair & 6 & 3173 & 139 & 2648 & 370 & 1.59\\ 
Arm & 6 & 507 & 99 & 291 & 196 & 0.52\\ 
Back & 4 & 239 & 124 & 794 & 377 & 0.87\\ 
Base & 4 & 346 & 57 & 22 & 28 & 0.08\\ 
Head & 2 & 0 & 0 & 18 & 0 & 0.01\\ 
Seat & 3 & 452 & 136 & 560 & 282 & 0.68\\ 
Footrest & 3 & 0 & 0 & 18 & 0 & 0.01\\ 
Pedestal-B & 2 & 45&	1&	33&	3&	0.02 \\ 
Regular-B & 5 &	792&	71&	565&177&0.50 \\ 
Star-B & 3&	125&	20&	491&	40&	0.15 \\ 
Total & -& 5679 & 647 & 5440 & 1473 & 4.34 \\ 
\hline
\end{tabular}
\end{center}
\end{table}

==> tables/partnet_compare.tex <==
\begin{table}[t!]
\begin{center}
\caption{Comparison for different methods to pass human verification on test set of PartNet.}
\label{tab:partnet_comparison}
\begin{tabular}{ |c|c|c|c|c|c|c| } 
\hline
 & Methods & PV & FV & PV/M & PM & T \\
\hline
\multirow{3}{3em}{Chair} &PartNet & - & - & 3657 & 3004 & 11.17\\ 
&NGSP & - & - & 4595 & 2066 & 8.36\\
&Ours & 5679 & 647 & 5440 & 1473 & 4.34\\ 
\hline
\multirow{3}{3em}{Table} &PartNet & - & - & 1785 & 3590 & 12.01\\ 
&NGSP & - & - & 2532 & 2843 & 9.86\\
&Ours &4473& 511 & 4541 & 1493 & 4.41\\ 
\hline
\multirow{3}{3em}{Lamp} &PartNet & - & - & 1441&	2323& 7.86
\\ 
&NGSP & - & - & 1873 &	1891 &	6.62\\
&Ours & 1209&	344	& 2359 &	857 & 2.16\\ 
\hline
\multirow{3}{3em}{Cabinet} &PartNet & - & - & 2430 & 1961 & 9.64\\ 
&NGSP & - & - & 3092 & 1357 & 7.28 \\
&Ours & 1450 & 451 & 3145 & 1267 & 3.87\\ 
\hline

\end{tabular}
\end{center}
\end{table}

==> tables/partnet_new.tex <==
\begin{table}[t!]
\begin{center}
\caption{Labeling time comparison against George et al.~[5]}
\label{tab:partnet_new}
\begin{tabular}{ l|c|c|c|c } 
\hline
 & Chair & Table & Lamp & Cabinet \\
\hline
George et al.~[5] & 10.39	& 13.47 & 9.83 & 8.27\\
\hline
HAL3D & {\bf 4.34} & {\bf4.41} & {\bf3.87} & {\bf2.16} \\
\hline
\end{tabular}
\end{center}
\vspace{-15pt}
\end{table}
